A remark on the Tate conjecture

The Tate conjecture has two parts: an assertion (S) about semisimplicity of Galois representations, and an assertion (T) which says that every Tate class is algebraic. We show that in characteristic 0, (T) implies (S). In characteristic p an analogous result is true under stronger assumptions.

==> BMmacs <==
\catcode`\@=11
\def\hexnumber@#1{\ifcase#1 0\or1\or2\or3\or4\or5\or6\or7\or8\or9\or
        A\or B\or C\or D\or E\or F\fi }

%%  Blackboard bold and msa fonts
%%
\font\tenmsa=msam10  \font\tenmsb=msbm10
\font\eightmsa=msam8 \font\eightmsb=msbm8
\font\sevenmsa=msam7 \font\sevenmsb=msbm7
\font\sixmsa=msam6   \font\sixmsb=msbm6
\font\fivemsa=msam5  \font\fivemsb=msbm5
\newfam\msafam
\textfont\msafam=\tenmsa  \scriptfont\msafam=\sevenmsa
  \scriptscriptfont\msafam=\fivemsa
\edef\msa@{\hexnumber@\msafam}
\newfam\msbfam
\textfont\msbfam=\tenmsb  \scriptfont\msbfam=\sevenmsb
  \scriptscriptfont\msbfam=\fivemsb
\edef\msb@{\hexnumber@\msbfam}
\def\Bbb{\ifmmode\let\next\Bbb@\else
        \def\next{\errmessage{Use \string\Bbb\space only in math
mode}}\fi\next}
\def\Bbb@#1{{\Bbb@@{#1}}}
\def\Bbb@@#1{\fam\msbfam#1}
%%
%%  RSFS
%%
\font\teneusm=rsfs10
\font\seveneusm=rsfs7
\font\fiveeusm=rsfs5
\newfam\eusmfam
\textfont\eusmfam=\teneusm  \scriptfont\eusmfam=\seveneusm
  \scriptscriptfont\eusmfam=\fiveeusm
\edef\eusm@{\hexnumber@\eusmfam}
\def\euscr{\ifmmode\let\next\euscr@\else
  \def\next{\errmessage{Use \string\euscr\space only in math mode}}\fi\next}
\def\euscr@#1{\fam\eusmfam#1}
%%
%%      sans serif (sf)
%%
\font\tensf=cmss10
\font\eightsf=cmss8
\font\sevensf=cmss7
\font\sixsf=cmss6
\font\fivesf=cmss5
\newfam\sffam
\textfont\sffam=\tensf  \scriptfont\sffam=\sevensf
  \scriptscriptfont\sffam=\fivesf
\def\hexnumber@#1{\ifcase#1 0\or1\or2\or3\or4\or5\or6\or7\or8\or9\or
        A\or B\or C\or D\or E\or F\fi }
\edef\sf@{\hexnumber@\sffam}
\def\sf{\let\next\sf@\next}
\def\sf@#1{\fam\sffam#1}
%%
\mathchardef\square="0\msa@03
\catcode`\@=12

%%
%% Fonts for 8-point
%%
\font\eightrm=cmr8  \font\sixrm=cmr6
\font\eighti=cmmi8  \font\sixi=cmmi6
\font\eightsy=cmsy8 \font\sixsy=cmsy6
\font\eightbf=cmbx8 \font\sixbf=cmbx6
\font\eighttt=cmtt8
\font\eightit=cmti8
\font\eightsl=cmsl8
\font\eighteusm=rsfs7 scaled\magstep1
\font\sixeusm=rsfs5 scaled\magstep1
%%
\catcode`@=11
\newskip\ttglue
\def\eightpoint{\def\rm{\fam0\eightrm}% switch to 8-point type
  \textfont0=\eightrm \scriptfont0=\sixrm \scriptscriptfont0=\fiverm
  \textfont1=\eighti  \scriptfont1=\sixi  \scriptscriptfont1=\fivei
  \textfont2=\eightsy \scriptfont2=\sixsy \scriptscriptfont2=\fivesy
  \textfont3=\tenex   \scriptfont3=\tenex \scriptscriptfont3=\tenex
  \textfont\itfam=\eightit  \def\it{\fam\itfam\eightit}%
  \textfont\slfam=\eightsl  \def\sl{\fam\slfam\eightsl}%
  \textfont\ttfam=\eighttt  \def\tt{\fam\ttfam\eighttt}%
  \textfont\bffam=\eightbf  \scriptfont\bffam=\sixbf
    \scriptscriptfont\bffam=\fivebf  \def\bf{\fam\bffam\eightbf}%
  \textfont\msafam=\eightmsa \scriptfont\msafam=\sixmsa
    \scriptscriptfont\msafam=\fivemsa
  \textfont\msbfam=\eightmsb \scriptfont\msbfam=\sixmsb
    \scriptscriptfont\msbfam=\fivemsb \def\Bbb{\fam\msbfam\eightmsb}%
 \textfont\eusmfam=\eighteusm \scriptfont\eusmfam=\sixeusm
    \scriptscriptfont\eusmfam=\fiveeusm
\def\euscr{\fam\eusmfam\eighteusm}%
  \tt \ttglue=.5em plus.25em minus.15em
  \normalbaselineskip=10pt
  \setbox\strutbox=\hbox{\vrule height7pt depth2pt width0pt}%
  \let\sc=\sixrm \let\big=\eightbig \normalbaselines\rm}
\def\eightbig#1{{\hbox{$\textfont0=\ninerm\textfont2=\ninesy
  \left#1\vbox to6.5pt{}\right.\n@space$}}}
\catcode`@=12

%% fonts for the title
%%
\font\namefont=cmr12
\font\byfont=cmti12
\font\titlefont=cmbx12

%% PAGE SIZE and PAGE LAYOUT:
%%
\hsize16truecm
\vsize23.5truecm
\normalbaselineskip=14pt
\normalbaselines

%% used for labels of references:
%%
\newcount\referno
\def\refno{\number\referno}
\def\bibitem#1{\advance\referno by1\definexref{#1}{\refno}{}\item{\hbox to 1.6em{{\rm [\refno]}\hfill}}}

\def\stretcharrow{\mathop{\hbox to 15pt{\rightarrowfill}}}
\def\mapright#1{\mathrel{\stretcharrow\limits^{\;\,#1\;\;}}}

%%  Blackboard Bold
%%
\def\mQ{{\Bbb Q}}
\def\mZ{{\Bbb Z}}
\def\Ql{\mQ_\ell}
\def\Zl{\mZ_\ell}

%%  Script letters:
%%
\def\cG{{\euscr G}}
\def\cT{{\euscr T}}

%%  "operator names"
%%
\def\Alt{{\rm Alt}}
\def\CH{{\rm CH}}
\def\Gal{{\rm Gal}}
\def\GL{{\rm GL}}
\def\Ker{{\rm Ker}}
\def\Spec{{\rm Spec}}
\def\Tate{\cT}
\def\mot{{\rm mot}}
\def\hom{{\rm hom}}
\def\num{{\rm num}}

%% some categories:
%%
\def\Mot{{\sf Mot}}
\def\Rep{{\sf Rep}}

%% fields:
%%
\def\Kbar{{\bar{K}}}
\def\Qbar{{\overline{\mQ}}}

\def\QED{\unskip\nobreak\hfill\hbox{$\mskip 9mu minus 5mu \square$}}

